On Coresets for Fair Clustering in Metric and Euclidean Spaces and Their Applications

Fair clustering is a constrained variant of clustering where the goal is to partition a set of colored points, such that the fraction of points of any color in every cluster is more or less equal to the fraction of points of this color in the dataset. This variant was recently introduced by Chierichetti et al. [NeurIPS, 2017] in a seminal work and became widely popular in the clustering literature. In this paper, we propose a new construction of coresets for fair clustering based on random sampling. The new construction allows us to obtain the first coreset for fair clustering in general metric spaces. For Euclidean spaces, we obtain the first coreset whose size does not depend exponentially on the dimension. Our coreset results solve open questions proposed by Schmidt et al. [WAOA, 2019] and Huang et al. [NeurIPS, 2019]. The new coreset construction helps to design several new approximation and streaming algorithms. In particular, we obtain the first true constant-approximation algorithm for metric fair clustering, whose running time is fixed-parameter tractable (FPT). In the Euclidean case, we derive the first $(1+\epsilon)$-approximation algorithm for fair clustering whose time complexity is near-linear and does not depend exponentially on the dimension of the space. Besides, our coreset construction scheme is fairly general and gives rise to coresets for a wide range of constrained clustering problems. This leads to improved constant-approximations for these problems in general metrics and near-linear time $(1+\epsilon)$-approximations in the Euclidean metric.

==> other-temp.tex <==
\section{Algorithms for Other Clustering Problems}
\label{sec:others}
We note that the algorithms for fair clustering in general metrics suggest a generic algorithm for any clustering problem with constraints, such that the constraints can be represented by a set of matrices. Here we state this algorithm. Let $\cd$ be the set of all possible distinct distances. Also, let $D_{\min}$ and $D_{\max}$ be the minimum and maximum distances in $\cd$, respectively. This algorithm has the following steps. 

\begin{itemize}
 \item Compute a universal coreset $W$. 
 \item For every pair of tuples $(l_1$, \ldots, $l_k)$ and $(R_1$, \ldots, $R_k)$ such that $l_i \in W$ for all $i$ and $R_j\in \cd$ for all $j$, do the following. 
 \begin{itemize}
  \item Select a set $C=\{c_1,\ldots,c_k\}$ of centers such that $c_i\in F$ and $d(l_i,c_i)\in [R_i,(1+\epsilon)R_i]$ for all $i$. If no such set $C$ exists, probe the next choice. 
  \item Find an assignment of the points in $P$ to the centers in $C$ of the minimum cost that satisfies the respective clustering constraints (assignment problem). 
 \end{itemize}
\item Return the set of centers and the assignment that minimizes the cost over all choices. 
\end{itemize}

From the analysis for fair clustering, we have the following theorem. 

\begin{theorem}\label{th:framework}
 Consider any clustering problem with constraint $K$, such that the constraint can be represented by a set of matrices, and suppose the aspect ratio $D_{\max}/D_{\min}$ is bounded by $\Delta$ for all instances. Moreover, suppose the universal coreset can be computed in $T_1(n,k,\ell)$ time and the assignment problem for the clustering problem can be solved in $T_2(n,k)$ time. Then one can obtain, w.h.p, a $(3+\epsilon)$- (resp. $(9+\epsilon)$-) approximation for $k$-median (resp. $k$-means) with constraint $K$ in time $T_1(n,k,\ell)+(\epsilon^{-1}k\Gamma\log (n+\Delta))^{O(k)}\cdot T_2(n,k)$.  
\end{theorem}

From the above theorem, it is sufficient to (i) show that the aspect ratios of instances are bounded and (ii) design an efficient algorithm for the assignment problem, to obtain constant approximations for a clustering problem with constraints. We will use this theorem on various clustering problems. 

For the Euclidean version of clustering problems with constraints, we have the following generic algorithm. 

\begin{itemize}
 \item Compute a universal coreset $W$. 
 \item Apply the algorithm mentioned in Proposition \ref{proposition:constrained} to find the list $\mathcal{L}$ of candidate sets of centers.   
 \item For every set $C=\{c_1,\ldots,c_k\}$ of centers in $\mathcal{L}$, do the following. 
 \begin{itemize}
  \item Find an assignment of the points in $W$ to the centers in $C$ of the minimum cost that satisfies the respective clustering constraints (assignment problem). 
 \end{itemize}
\item Let $C'$ be the set of centers that minimizes the cost over all choices. Find an assignment of the points in $P$ to the centers in $C'$ of the minimum cost that satisfies the respective clustering constraints. 
\end{itemize}

From the analysis for fair clustering and Proposition \ref{proposition:constrained}, we know that $C'$ is an approximately optimal set of centers with constant probability. By repeating step 3 of the above algorithm $O(\log n)$ times,  we obtain this w.h.p. Hence, we have the following theorem. 

\begin{theorem}\label{th:frameworkRd}
 Consider any Euclidean clustering problem with constraint $K$, such that the constraint can be represented by a set of matrices. Moreover, suppose the universal coreset can be computed in $T_1(n,k,\ell,d)$ time and the assignment problem for the clustering problem can be solved in $T_2(n,k)$ time for $n$ points. Then one can obtain, w.h.p, a $(1+\epsilon)$-approximation for $k$-median (resp. $k$-means) with constraint $K$ in time $T_1(n,k,\ell,d)+2^{\tilde{O}(k/\epsilon^{O(1)})}\cdot \log n\cdot (d^2\Gamma(\epsilon^{-1}k\log n)^{O(1)}+T_2(|W|,k))+T_2(n,k)$.  
\end{theorem}

From the above theorem, it is sufficient to  design an efficient algorithm for the assignment problem, to obtain constant approximations for a clustering problem with constraints. In the following, we will use this theorem on various clustering problems. 

\subsection{Lower-Bounded Clustering}
In the lower-bounded clustering problem, we are given a lower bound parameter $L$ and the size of each cluster must be at least $L$. In the Euclidean version of the problem the set of points $P\subset \mathbb{R}^d$ and the set of centers $F=\mathbb{R}^d$. 

First, we note that the lower bound constraint can be represented by a set of $k\times 1$ column matrices such that each of the entries is at least $L$ and at most $n$. 

To apply Theorem \ref{th:framework}, we need two things as mentioned before. To show the bounded aspect ratio, we can use any $O(1)$-approximation for the problem. Then, we can argue in the same way as we did for fair clustering. The assignment problem for lower-bounded clustering can be modelled as a minimum cost network flow problem that can be solved in polynomial time. Indeed, the modelling is similar to the one in the proof of Lemma \ref{lemma:restore_assignment}. Let $P'$ be the input set of $n$ points and $C$ be the set of $k$ centers. Each point $p$ has a weight $w(p)$ that we need to assign to the centers in $C$. We construct a bipartite network where on one side we have the $n$ points of $P'$ and on the other side the $k$ centers of $C$ and an additional node $w$. Source $s$ is connected to all points of $P'$. Sink $t$ is connected to all centers through edges of capacity $L$. $t$ is also connected to $w$ through an edge of capacity $n-kL$. $w$ is connected to all points through an edge. The cost of the edges between points and centers are their respective distances times their weight. The cost between a point $p$ and $w$ is $d(p,C)$. The idea is to route $L$ flow to each center and $n-kL$ flow to $w$. This is equivalent to assigning at least $L$ points to each center using the minimum cost and assigning the remaining points to their closest neighbor in $C$. We also scale the distances, as mentioned in the proof of Lemma \ref{lemma:restore_assignment}. Then, the cost of the minimum cost flow in this network (with $n$ flow) is a $(1+\epsilon)$-approximation of the minimum assignment cost. Hence, by Proposition \ref{proposition_unbalanced_flow}, the assignment problem in this case can be solved in time $nk^2\epsilon^{-O(1)}\log n$. Hence, the constant approximations follow for this problem in general metrics in time $$O(nk)+(\epsilon^{-1}k\log n)^{O(k)}nk^2\epsilon^{-O(1)}\log n=(\epsilon^{-1}k\log n)^{O(k)}n=(k/\epsilon)^{O(k)}n^{O(1)}.$$   

From the above discussion, one can also apply Theorem \ref{th:frameworkRd}. The time complexity of the assignment problem for coreset points is $|W|k^2\epsilon^{-O(1)}\log |W|=(\epsilon^{-1}k\log n)^{O(1)}$. Hence, we obtain $(1+\epsilon)$-approximation for the Euclidean version in time $$O(nkd)+2^{\tilde{O}(k/\epsilon^{O(1)})}\cdot d^2(\epsilon^{-1}k\log n)^{O(1)}+nk^2\epsilon^{-O(1)}\log n=2^{\tilde{O}(k/\epsilon^{O(1)})}d^2(\log n)^{O(1)}+dk^2\epsilon^{-O(1)}n\log n.$$

\subsection{Capacitated Clustering}
Here we study the Euclidean capacitated clustering where the set of points $P\subset \mathbb{R}^d$ and the set of centers $F=\mathbb{R}^d$. Additionally, we are given a capacity parameter $U$ and the size of each cluster must be at most $U$. 

First, we note that the capacity constraint can be represented by a set of $k\times 1$ column matrices such that each of the entries is at least $0$ and at most $U$. 

Now, the assignment problem for capacitated clustering can be modelled as a minimum cost network flow problem that can be solved in polynomial time. Again, the modelling is similar to the one in the proof of Lemma \ref{lemma:restore_assignment}. We construct a complete bipartite network where on one side we have the $n$ points of $P$ and on the other side the $k$ centers of $C$. Source $s$ is connected to all points of $P$. Sink $t$ is connected to all centers with edges of capacity $U$. The cost of the edges between points and centers are their respective distances. We also scale the distances, as mentioned in the proof. Then, the cost of the minimum cost flow in this network (with $n$ flow) is a $(1+\epsilon)$-approximation of the minimum assignment cost. We note that one can assume that the aspect ratio of the input instance is bounded by $(n/\epsilon)^{O(1)}$ \cite{Cohen-AddadL19}. Hence, by Proposition \ref{proposition_unbalanced_flow}, the assignment problem in this case can be solved in time $nk^2\epsilon^{-O(1)}\log n$. A $(1+\epsilon)$-approximation follows for the Euclidean version in time $$O(nkd)+2^{\tilde{O}(k/\epsilon^{O(1)})}\cdot d^2(\epsilon^{-1}k\log n)^{O(1)}+nk^2\epsilon^{-O(1)}\log n=2^{\tilde{O}(k/\epsilon^{O(1)})}d^2(\log n)^{O(1)}+dk^2\epsilon^{-O(1)}n\log n.$$


\subsection{$\ell$-Diversity Clustering}
In the $\ell$-Diversity clustering problem, $P=\cup_{i=1}^{\tilde{n}} P_i$ is a set of $n$ colored points such that all points in $P_i$ have the same color, and each
cluster must have no more than a fraction $1/\ell$ (for some
constant $\ell > 1$) of its points sharing the same color. Thus, for each cluster $A$ and $i\in [\ell]$, $|A\cap P_i|\le |A|/\ell$. We note that each point can have only one color. Ding and Xu~\cite{ding2020unified} gave a $(1+\epsilon)$-approximation for this problem in $\mathbb{R}^d$ with time complexity $O(n^2(\log n)^{k+2}(t+1)^kd)$, where $t=\max_{1\le i\le \tilde{n}} |P_i|$. 

We note that $\ell$-Diversity clustering is a special case of $(\alpha,\beta)$-fair clustering without the lower bound constraints involving parameter $\beta$, and $\alpha_i=1/\ell$ for all $i$. Thus, we obtain algorithms for this problem with bounds same as for $(\alpha,\beta)$-fair clustering, including a $(1+\epsilon)$-approximation that significantly improves the time complexity of the one in \cite{ding2020unified}.     


\subsection{Chromatic Clustering}
In chromatic clustering, again $P=\cup_{i=1}^{\tilde{n}} P_i$ is a set of $n$ colored points such that all points in $P_i$ have the same color, and each cluster contains at most one point from $P_i$ for each $i$. Ding and Xu~\cite{ding2020unified} obtained a linear time $(1+\epsilon)$-approximation for this problem in $\mathbb{R}^d$. To the best of our knowledge the metric version of the problem was not studied before. Thus, we give the first constant approximation for this version. 

First, we note that the chromatic constraint can be represented by a set of $k\times \ell$  matrices with 0/1 entries. 

Ding and Wu~\cite{ding2020unified} showed that the assignment problem for chromatic clustering can be modelled as a bipartite matching problem that can be solved in $O(k^3n)$ time. However, it is not clear how to bound the aspect ratio for this problem. Hence, the constant approximations follow for this problem in general metrics in time $O(nk)+(\epsilon^{-1}k\ell\log (n+\Delta))^{O(k)}n$.   


